Hierarchical Composable Optimization of Web Pages

The process of creating modern Web media experiences is challenged by the need to adapt the content and presentation choices to dynamic real-time fluctuations of user interest across multiple audiences. We introduce FAME - a Framework for Agile Media Experiences - which addresses this scalability problem. FAME allows media creators to define abstract page models that are subsequently transformed into real experiences through algorithmic experimentation. FAME's page models are hierarchically composed of simple building blocks, mirroring the structure of most Web pages. They are resolved into concrete page instances by pluggable algorithms which optimize the pages for specific business goals. Our framework allows retrieving dynamic content from multiple sources, defining the experimentation's degrees of freedom, and constraining the algorithmic choices. It offers an effective separation of concerns in the media creation process, enabling multiple stakeholders with profoundly different skills to apply their crafts and perform their duties independently, composing and reusing each other's work in modular ways.

==> Appendices.tex <==
\appendix

\section{Layout HTML Example}\label{app: layout html}

%\parbox[b]{10cm}{
\begin{verbatim}
<html>
 <body>
  <table label="layout">
   <tr label="header" />
   <tr label="body">
    <td label="westRegtion" />
    <td label="centerRegtion">
     <table>
      <tr label="centerUpRegion">
       <td></td>
      </tr>
      <tr label="centerButtomRegion">
       <td></td>
      </tr>
     </table>
    </td>
    <td label="eastRegtion">
     <table>
      <tr label="East1Region">
       <td></td>
      </tr>
      <tr label="East2Region">
       <td></td>
      </tr>
      <tr label="East3Region">
       <td></td>
      </tr>
      <tr label="East4Region">
       <td></td>
      </tr>
     </table>
    </td>
   </tr>
  </table>
 </body>
</html>
\end{verbatim}

\section{POTL Example}\label{app: POTL file}

\begin{verbatim}
<layout label="MainPage">
 <apl:constraints id="MainPageConstraints">
  <region label="YahooHeader">
   <module label="YahooHeaderModule">
    <source label="YahooHeaderSource">
     <apl:operator id="yahooHeaderOperator" 
handler="YahooHeaderSearcherChain" />
    </source>
    <renderer label="YahooHaederRendererHandler" />
   </module>
  </region>
  <region label="YahooSitesRegion">
   <module label="YahooSitesModule">
    <source label="YahooSiteSource">
     <apl:constraints id="YahooSitesConstraints">
     <!-- Mapping 18 items out of 30 to 18 positions -->
       <apl:map id="YahooSiteMap" 
handler="SiteSelectorSearcherChain">
        <apl:operator id="yahooSiteOperator" 
handler="YahooSiteSearcherChain">
         <property key="number of regions" value="18" />
         <property key="number of items" value="30" />
         </apl:operator>
          </apl:map>
           <apl:constraint id="YahooSiteConstraint1">
            <![CDATA[function isValid(query, executionMap) {
            // Mail and messenger sites can't be in 
            // consecutive positions.
            }]]>
           </apl:constraint>
           <apl:constraint id="YahooSiteConstraint2">
            <![CDATA[function isValid(query, executionMap) {
            // If travel site is included then 
            // weather is included as well.
            }]]>
           </apl:constraint>
           <apl:constraint id="YahooSiteConstraint3">
            <![CDATA[function isValid(query, executionMap) {
            // Mail is always mapped to the first position.
            }]]>
           </apl:constraint>
          </apl:constraints>
         </source>
         <renderer label="YahooSiteRendererHandler" />
        </module>
       </region>
       <region label="TodayRegion">
        <module label="TodayModule">
         <source label="TodaySource">
          <apl:constraints id="TodayConstraints">
          <!-- Mapping 4 items out of 500 to 4 place holders -->
           <apl:map id="TodayMap" 
handler="HotItemSearcherChain">
            <region label="news1">
             <apl:position id="news1" />
            </region>
            <region label="News2">
             <apl:position id="news2" />
            </region>
            <region label="News3">
             <apl:position id="news3" />
            </region>
            <region label="News4">
             <apl:position id="news4" />
            </region>
            <apl:operator id="NewsOperator" 
handler="NewsSearcherChain">
           </apl:operator>
          </apl:map>
          <apl:constraint id="TodayConstraint1">
           <![CDATA[function isValid(query, executionMap) {
                    // No more than 2 sport news items.
                    }]]>
          </apl:constraint>
          <apl:constraint id="TodayConstraint2">
           <![CDATA[function isValid(query, executionMap) {
           // At least one geo local news item (relates to the geographical 
           // location of the user).
           }]]>
          </apl:constraint>
          <apl:constraint id="TodayConstraint3">
           <![CDATA[function isValid(query, executionMap) {
           // The first news item must be less than 2 hours old.
           }]]>
          </apl:constraint>
         </apl:constraints>
        </source>
        <renderer label="TodayRendererHandler" />
       </module>
      </region>
      <region label="TrendingNowRegion">
       <module label="TrendingNowModule">
        <source label="TrendingNowSource">
         <apl:constraints id="TrendingNowConstraints">
         <!-- Mapping 10 items out of 300 to 10 place holders -->
           <apl:map id="TrendingNowMap" 
handler="InorderMapSearcherChain">
            <apl:operator id="TrendingNowOperator" 
handler="TrendingNowSearcherChain">
             <property key="number of regions" value="10" />
             <property key="number of items" value="300" />
            </apl:operator>
           </apl:map>
           <apl:constraint id="No more of 2 trends of the same category contencuse">
            <![CDATA[function isValid(query, executionMap) {
             // No more than 3 celeb related trends.
            }]]>
           </apl:constraint>
           <apl:constraint id="long queries in the five last positions">
            <![CDATA[function isValid(query, executionMap) {
            // Trends with more than 2 words can't 
            // be placed in the same row
            }]]>
           </apl:constraint>
          </apl:constraints>
         </source>
         <renderer label="TrendingNowRendererHandler" />
        </module>
      </region>
      <region label="DisplayAds">
       <module label="DisplayAdsModule">
        <source label="DisplayAdsSource">
         <apl:operator id="DisplayAdsOperator" 
handler="DisplayAdsSearcherChain" />
        </source>
        <renderer label="DisplayAdsRendererHandler" />
       </module>
      </region>
      <region label="VeritcalHeadlines">
       <module label="VeritcalHeadlinesModule">
        <source label="VeritcalHeadlinesSource">
         <apl:operator id="VeritcalHeadlinesOperator" handler="VeritcalHeadlinesSearcherChain" />
        </source>
        <renderer label="VeritcalHeadlinesRendererHandler" />
       </module>
      </region>
      <region label="LatestVideo">
       <module label="LatestVideoModule">
        <source label="LatestVideoSource">
         <apl:operator id="LatestVideoOperator" 
handler="LatestVideoSearcherChain" />
        </source>
        <renderer label="LatestVideoRendererHandler" />
       </module>
      </region>
      <region label="YahooVertical">
       <module label="YahooVerticalModule">
        <source label="YahooVerticalSource">
         <apl:choice id="ImageColorChoice">
          <apl:alternative id="vertical1Alternativ">
           <apl:operator id="vertical1" 
handler="VerticalInfoSearchChain">
            <proprty key="verticalId" value="cars" />
           </apl:operator>
          </apl:alternative>
          <apl:alternative id="vertical2Alternativ">
           <apl:operator id="vertical2" 
handler="VerticalInfoSearchChain">
            <proprty key="verticalId" value="jobs" />
           </apl:operator>
          </apl:alternative>
          <apl:alternative id="vertical3Alternativ">
           <apl:operator id="vertical3" 
handler="VerticalInfoSearchChain">
            <proprty key="verticalId" value="games" />
           </apl:operator>
          </apl:alternative>
         </apl:choice>
        </source>
        <renderer label="YahooVerticalRendererHandler" />
       </module>
      </region>
     </apl:constraints>
    </layout>
   </apl:template>
\end{verbatim}


==> conc.tex <==
\section{Conclusions and Future Work}
\label{sec:conc}

This work presented \APLcomma a framework for creating agile Web media experiences through
algorithmic experimentation and optimization. The input to \APL are page instantiation requests
expressed by logical page models, which define (1) dynamic data to be fetched,
(2) degrees of freedom to algorithmically experiment with,
subject to (3) editorial constraints, toward optimization of the page for user experience and business goals.
During page instantiation, \APLs execution engine orchestrates various algorithmic plug-ins, which
collectively morph the logical page model into a concrete page by resolving the model's degrees of freedom.

%redundant paragraph
\comment{
We demonstrated \APLs page model and the transformations it undergoes when morphing into a concrete page
on a major Web media page. This included the fetching of dynamic data, definition and subsequent resolution
of degrees of freedom subject to constraints, and the addition of instrumentation directives.
}

\APL improves upon existing systems that perform multivariate optimization of Web pages in several aspects. 
It incorporates fetchers which import dynamic content into its page models in real time. 
It is further designed for hierarchical optimization of the page, meaning that it implicitly defines a workflow
of decisions to be made and content to be fetched. In particular, this allows pages to be optimized given the
attributes of the content that is available at page instantiation time.
While \APLcomma like previous systems, defines multiple degrees of freedom to be resolved on its pages,
it differs from those systems in that it uses a mechanism of constraints that avoids serving page instances 
with conflicting resolutions.
Finally, \APL is an open platform, and defines interfaces and extension points that allow multiple optimization
algorithms to be plugged in, each resolving specific portions of the page. Related work in Section~\ref{sec:related}
surveyed several reinforcement learning techniques %that have been applied to Web media pages, and 
which are natural plug-ins into \APL.

An important consequence of \APLs architecture is that the building blocks of its page models - hierarchical structure,
fetchers, resolvers and constraints - naturally map to the responsibilities of different stakeholders in the online
media serving pipeline. The architectural modularity enables a separation of concerns that allows people of different
roles and skill sets -- UED specialists, media editors, product owners and optimization experts -- to work independently
and then compose and reuse their artifacts in an agile manner.

Future work will shift the focus from the framework and platform aspect onto evaluations of complex optimization scenarios,
where multiple resolvers implementing different learning algorithms are composed hierarchically and are orchestrated
by the platform to reach well-performing whole-page operating points with respect to a spectrum of target functions.


==> disc.tex <==
\section{Discussion}
\label{sec:disc}
This section is currently a placeholder for discussion of various points that don't naturally fit in the other sections.
I assume that as the paper evolves, we'll have more topics for this section. Currently, one topic to think about is whether 
we can say something about framework's loss of optimization due to the decomposition of the decisions.

==> introduction.tex <==
\section{Introduction}
Digital media websites have mainly grown out of traditional media outlets, e.g. TV and printed press.
Accordingly, such sites produce their pages in a process resembling traditional media, i.e. 
through an editorial board that decides on the various aspects of the page -- its layout, which content
items (including ads) to place where in the layout, and how to render (or format) the content. 
%
Editors of printed and broadcast media are typically senior journalists, who mostly apply human judgment,
intuition and experience in creating their editions. However, two gating factors limit their ability to
optimize, in a methodological manner, the product they put in front of their audience.

First, print editors have no way of tracking (other than through, perhaps, small focus groups) 
how their product was consumed and how it ``performed'', i.e. which stories, sections or ads 
resonated well with the readership/viewership and which didn't. Circulation and ratings trends
take many weeks to develop, and are difficult to attribute to any specific decisions 
made by the editors. In contrast, through proper instrumentation, digital media editors 
can get immediate feedback on the consumption of their product. It is easy to track in real-time 
the number of times each story (or ad) was clicked, each video played, and each survey answered. 
Tracking unique visitors and repeat visitors in an accurate manner over any time period is
also possible. Unlike their counterparts from the press, editors of online media have no lack 
of data -- on the contrary, they perhaps have too much data to humanly reason about.

A second major difference between printed and broadcast media and online media revolves around 
the concept of an ``edition''. Printed media outputs editions at fixed intervals, e.g. daily 
or weekly, and prints a limited number of different versions per edition (e.g. editions may vary 
slightly between locales). Television programs are also produced at a regular pace, with minor 
variability. In contrast, online media isn't bound to the concept of editions, and content can 
rotate in and out of a Web page in real time. Lifetimes of content items vary, i.e. some items
can remain served much longer than others. Furthermore, the number of different served versions 
of a page may, theoretically, equal the number of users to whom it was served.

Obviously, editorial attention does not scale to support the shift from a small discrete space of
editions to a large continuum. Human analysis of complex instrumentation is also not scalable. 
With proper automation, however, online media can tap the ability to produce a continuum of editions to 
{\em experiment} with a huge variety of generated pages. The power of interaction instrumentation and 
the resulting usage statistics can then be leveraged to optimize the media experience - namely, choose 
the settings that produce the most favorable experience at every point in time. 

In recent years, reinforcement learning has been applied in various contexts to optimize digital media 
in the sense described above, mainly by tapping click-through rates. Examples include optimizing search 
results ranking \cite{RTUF-learning2010,InterleavedBuckets} and main story optimization \cite{COKE2009,COKE2008}. 
Whereas the above works mainly revolved around optimizing content, other efforts leveraged user interactions
to optimize presentation, e.g. layout of content on mobile devices \cite{MobileLayout2004}.
These efforts demonstrated that algorithmic optimization of media can outperform editorial 
decisions and intuitions.

We envision that editors of future media sites will oversee their product at a high level,
delegating many functions to algorithmic machinery, to keep up with scalability challenges.
They will leverage experience and intuition to
define the desired experiences in abstract terms, through {\em logical page models}. 
Rather than fully specifying the page, these models will include {\em degrees of freedom}
on its layout, content and formatting, {\em constraints} on how those degrees of freedom may 
be jointly resolved, and the {\em target function} to pursue. For example, degrees of freedom 
may include specifying a large content pool from which several stories are to be selected, 
choosing from among several layouts, and choosing formatting or algorithmic configuration parameters. 
Constraints may be imposed on the joint resolutions of the degrees of freedom, thus introducing 
dependencies between those resolutions. Target functions may factor in user engagement (click-through 
rates, repeat visits, etc.) as well as monetization aspects. The actual optimization of the page,
within the parameters defined by the editors, will be algorithmic.

This paper introduces \APL -- a Framework for Agile Media Experiences. 
We present the vision and prototype of the system, parts of which are already in production 
at a major Internet portal. \APL defines a hierarchical logical model for describing 
complex self-optimizing web pages. This model allows a fine-grained interplay between 
algorithmic decisions and editorial control. \APL allows independent plug-ins to optimize various 
decisions on the page, and orchestrates those plug-ins so that their joint output will satisfy 
the constraints while performing well in the target function. Essentially, the \APL execution 
engine explores the space of possible page instantiations, attempting to converge to the best 
performing one. 

Our architecture emphasizes the decoupling and composability of all artifacts -- dynamic data 
sources, degrees of freedom, constraints and optimization plug-ins -- across multiple pages. 
Thus, the different stakeholders that participate in the media creation process can perform 
their roles in a mostly independent and repeatable fashion, while utilizing profoundly different
skill sets. To the best of our knowledge, no existing page optimization system achieves this 
level of separation-of-concerns, while capturing the complex structure of modern Web pages
as well as accommodating state-of-the-art optimization algorithms. 

The rest of this paper is organized as follows. Section~\ref{sec:players} describes the ecosystem 
of online media creation, and explains how the the \APL framework combines the efforts of the 
various stakeholders in agile creation of optimized media pages. Section~\ref{sec:related} 
surveys related work, and emphasizes our contributions. Section~\ref{sec:model} defines our 
logical page model, and specifies how degrees of freedom for experimentation are injected into 
the pages. Section~\ref{sec:constraints} extends the page model by adding constraints that 
enforce editorial validity of the result. Section~\ref{sec:execution} introduces the model 
execution engine. The \APL machinery applies algorithmic plug-ins to optimize the actual content and 
layout choices within the aforementioned degrees of of freedom, while adhering to the user-defined 
constraints. Section~\ref{sec:rtuf} describes \APLs infrastructure for collecting and harnessing
real-time user feedback, and Section~\ref{sec:conc} concludes the paper. 

==> outline.tex <==
Target conference: VLDB (Very Large Databases)
Target date: December 31
Title(??): Framework for Hierarchical Composable Optimization of Web Experiences

Hierarchical: Web pages are built from atomic data items (stories, links, pictures) that are packed into a hierarchy of higher level constructs like modules, frames, navigation bars, side bars/rails, etc. Each such construct is subject to optimization.

Composable: a Web experience contains many sub-problems, each perhaps optimized by a different algorithmic approach. The sub-problems tend to appear in many contexts, where in different contexts they are rolled up differently. We'd like to reuse Optimizers across experiences.

Optimization: here we should talk about types of target functions (interaction, monetization) and the fact that the target function may be parameterized in the problem being solved

Players (describe pre-framework and post-framework players, and who the framework replaces)
- ``User experience folks'' which design layouts (with degrees of freedom) and which give constraints
- ``Content editors'' which traditionally select content items to populate layout
- Optimization experts which tackle sub-problems and come up with algorithms to solve them
- framework, which allows all players above to virtually act together for a particular experience, where in practice the various players may have never met, never tailored their decisions to the common context, and don't even know who their artifacts are interacting with.


Execution model: bottom up resolution of XML, and how this supports many optimization algorithms (backtracking, branch and bound, beam search)

Story about constraints:
- At any level of the tree
- scope is subtree
- hints and conflicts
- This is not a SAT scenario, where we're looking for a very small set of satisfying assignments in an exponential search space. The typical case has a constant ratio of legal assignments. The system must operate in real-time, i.e. subsecond response times for http requests

Optimizers:
- Why iterators (intuition from Query Engines)
- Materialized vs. non-materialized iterators
- Hints and conflicts
- The runtime facade and the modeling (RTUF) facade

Shortcomings:
No ``live'' evaluation of quality
  - Can we say something about framework's loss of optimization due to the decomposition of the decisions
No evaluation of performance/SLA


Related work: ?????







